The Parsec-Scale Relationship Between I_CO and A_V in Local Molecular Clouds

We measure the parsec-scale relationship between integrated CO intensity (I_CO) and visual extinction (A_V) in 24 local molecular clouds using maps of CO emission and dust optical depth from Planck. This relationship informs our understanding of CO emission across environments, but clean Milky Way measurements remain scarce. We find uniform I_CO for a given A_V, with the results bracketed by previous studies of the Pipe and Perseus clouds. Our measured I_CO-A_V relation broadly agrees with the standard Galactic CO-to-H2 conversion factor, the relation found for the Magellanic clouds at coarser resolution, and numerical simulations by Glover & Clark (2016). This supports the idea that CO emission primarily depends on shielding, which protects molecules from dissociating radiation. Evidence for CO saturation at high A_V and a threshold for CO emission at low A_V varies remains uncertain due to insufficient resolution and ambiguities in background subtraction. Resolution of order 0.1 pc may be required to measure these features. We use this I_CO-AV relation to predict how the CO-to-H2 conversion factor (X_CO) would change if the Solar Neighborhood clouds had different dust-to-gas ratio (metallicity). The calculations highlight the need for improved observations of the CO emission threshold and HI shielding layer depth. They are also sensitive to the shape of the column density distribution. Because local clouds collectively show a self-similar distribution, we predict a shallow metallicity dependence for X_CO down to a few tenths of solar metallicity. However, our calculations also imply dramatic variations in cloud-to-cloud X_CO at subsolar metallicity.

==> icoav.tex <==
\begin{tabular}{llcc}
\hline \hline
Cloud & $A_V$ & $I_{\rm CO}$ \\ 
& (mag) & (K km s$^{-1}$) \\ 
\hline \hline
Aquila_South  &  0.25& $ 0.2 \pm  1.2$ \\
Aquila_South  &  0.50& $ 0.6 \pm  1.4$ \\
Aquila_South  &  0.75& $ 1.4 \pm  1.6$ \\
Aquila_South  &  1.00& $ 2.2 \pm  1.7$ \\
Aquila_South  &  1.25& $ 2.3 \pm  1.0$ \\
Aquila_South  &  1.50& $ 0.8 \pm  0.8$ \\
California  &  0.25& $ 0.7 \pm  1.6$ \\
California  &  0.50& $ 1.5 \pm  2.0$ \\
California  &  0.75& $ 2.7 \pm  2.1$ \\
California  &  1.00& $ 3.9 \pm  2.5$ \\
California  &  1.25& $ 5.1 \pm  2.9$ \\
California  &  1.50& $ 5.8 \pm  3.6$ \\
California  &  1.75& $ 6.7 \pm  4.2$ \\
California  &  2.00& $ 8.4 \pm  3.7$ \\
California  &  2.25& $ 8.8 \pm  4.0$ \\
California  &  2.50& $ 9.9 \pm  5.1$ \\
California  &  2.75& $12.0 \pm  4.0$ \\
California  &  3.00& $12.6 \pm  2.9$ \\
California  &  3.25& $11.4 \pm  2.4$ \\
California  &  3.50& $12.8 \pm  2.8$ \\
California  &  3.75& $13.6 \pm  1.6$ \\
California  &  4.00& $12.0 \pm  2.8$ \\
California  &  4.25& $13.4 \pm  2.8$ \\
California  &  4.50& $12.4 \pm  2.5$ \\
California  &  4.75& $13.0 \pm  1.6$ \\
California  &  5.00& $12.5 \pm  3.4$ \\
California  &  5.25& $13.5 \pm  2.0$ \\
California  &  5.50& $15.1 \pm  1.1$ \\
Camelopardalis  &  0.25& $ 0.2 \pm  1.3$ \\
Camelopardalis  &  0.50& $ 0.6 \pm  1.4$ \\
Camelopardalis  &  0.75& $ 1.5 \pm  1.6$ \\
Camelopardalis  &  1.00& $ 2.8 \pm  2.3$ \\
Canis_Major  &  0.25& $ 1.6 \pm  1.7$ \\
Canis_Major  &  0.50& $ 2.4 \pm  1.8$ \\
Canis_Major  &  0.75& $ 2.5 \pm  1.8$ \\
Canis_Major  &  1.00& $ 2.9 \pm  1.8$ \\
Canis_Major  &  1.25& $ 3.2 \pm  2.4$ \\
Canis_Major  &  1.50& $ 4.1 \pm  2.4$ \\
Canis_Major  &  1.75& $ 5.4 \pm  3.6$ \\
Canis_Major  &  2.00& $ 6.1 \pm  3.5$ \\
Canis_Major  &  2.25& $ 7.1 \pm  3.2$ \\
Canis_Major  &  2.50& $ 6.7 \pm  3.3$ \\
Canis_Major  &  2.75& $ 8.5 \pm  4.9$ \\
Canis_Major  &  3.00& $ 9.1 \pm  4.8$ \\
Canis_Major  &  3.25& $10.6 \pm  2.8$ \\
Canis_Major  &  3.50& $12.8 \pm  6.1$ \\
Canis_Major  &  3.75& $13.0 \pm  4.9$ \\
Canis_Major  &  4.00& $15.2 \pm  8.6$ \\
Canis_Major  &  4.50& $15.6 \pm  5.0$ \\
Canis_Major  &  5.25& $18.9 \pm  3.0$ \\
Canis_Major  &  5.50& $20.7 \pm  8.0$ \\
Cepheus_North  &  0.25& $ 2.2 \pm  1.7$ \\
Cepheus_North  &  0.50& $ 2.6 \pm  2.0$ \\
Cepheus_North  &  0.75& $ 3.6 \pm  2.1$ \\
Cepheus_North  &  1.00& $ 4.9 \pm  2.2$ \\
Cepheus_North  &  1.25& $ 6.8 \pm  2.9$ \\
Cepheus_North  &  1.50& $ 9.9 \pm  3.2$ \\
Cepheus_North  &  1.75& $11.9 \pm  3.5$ \\
Cepheus_North  &  2.00& $13.8 \pm  3.3$ \\
Cepheus_North  &  2.25& $14.9 \pm  3.9$ \\
Cepheus_North  &  2.50& $14.8 \pm  2.0$ \\
Cepheus_North  &  2.75& $15.6 \pm  2.7$ \\
Cepheus_North  &  3.00& $17.6 \pm  3.7$ \\
Cepheus_North  &  3.25& $18.2 \pm  3.2$ \\
Cepheus_North  &  3.50& $20.4 \pm  1.1$ \\
Cepheus_South  &  0.25& $ 1.3 \pm  1.0$ \\
Cepheus_South  &  0.50& $ 1.4 \pm  1.2$ \\
Cepheus_South  &  0.75& $ 1.5 \pm  1.2$ \\
Cepheus_South  &  1.00& $ 2.2 \pm  1.4$ \\
Cepheus_South  &  1.25& $ 2.6 \pm  1.7$ \\
Cepheus_South  &  1.50& $ 3.3 \pm  1.5$ \\
Cepheus_South  &  1.75& $ 4.7 \pm  2.3$ \\
Cepheus_South  &  2.00& $ 6.0 \pm  2.6$ \\
Cepheus_South  &  2.25& $ 8.1 \pm  3.0$ \\
Cepheus_South  &  2.50& $10.5 \pm  3.3$ \\
Cepheus_South  &  2.75& $11.8 \pm  2.2$ \\
Cepheus_South  &  3.00& $14.5 \pm  1.9$ \\
Cepheus_South  &  3.25& $16.4 \pm  2.8$ \\
Chamaeleon  &  0.25& $ 0.1 \pm  0.9$ \\
Chamaeleon  &  0.50& $ 0.7 \pm  1.1$ \\
Chamaeleon  &  0.75& $ 2.1 \pm  2.1$ \\
Chamaeleon  &  1.00& $ 3.8 \pm  2.5$ \\
Chamaeleon  &  1.25& $ 5.7 \pm  2.7$ \\
Chamaeleon  &  1.50& $ 6.9 \pm  2.3$ \\
Chamaeleon  &  1.75& $ 7.8 \pm  2.3$ \\
Chamaeleon  &  2.00& $ 8.7 \pm  3.0$ \\
Chamaeleon  &  2.25& $ 9.6 \pm  3.0$ \\
Chamaeleon  &  2.50& $10.2 \pm  2.7$ \\
Chamaeleon  &  2.75& $11.1 \pm  3.1$ \\
Chamaeleon  &  3.00& $10.3 \pm  2.6$ \\
Chamaeleon  &  3.25& $12.0 \pm  2.6$ \\
Chamaeleon  &  3.50& $12.4 \pm  3.0$ \\
Chamaeleon  &  3.75& $12.6 \pm  2.8$ \\
Chamaeleon  &  4.00& $12.3 \pm  2.7$ \\
Chamaeleon  &  4.25& $13.4 \pm  3.8$ \\
Chamaeleon  &  4.50& $12.2 \pm  2.2$ \\
Chamaeleon  &  4.75& $14.1 \pm  1.6$ \\
Gem_OB1  &  0.25& $ 1.4 \pm  1.4$ \\
Gem_OB1  &  0.50& $ 1.5 \pm  1.6$ \\
Gem_OB1  &  0.75& $ 1.9 \pm  1.6$ \\
Gem_OB1  &  1.00& $ 2.4 \pm  1.8$ \\
Gem_OB1  &  1.25& $ 3.2 \pm  2.0$ \\
Gem_OB1  &  1.50& $ 3.9 \pm  2.2$ \\
Gem_OB1  &  1.75& $ 4.6 \pm  2.9$ \\
Gem_OB1  &  2.00& $ 5.6 \pm  2.8$ \\
Gem_OB1  &  2.25& $ 6.3 \pm  3.5$ \\
Gem_OB1  &  2.50& $ 6.9 \pm  3.8$ \\
Gem_OB1  &  2.75& $ 8.4 \pm  3.9$ \\
Gem_OB1  &  3.00& $ 8.5 \pm  3.3$ \\
Gem_OB1  &  3.25& $ 9.3 \pm  3.5$ \\
Gem_OB1  &  3.50& $10.3 \pm  4.2$ \\
Gem_OB1  &  3.75& $11.7 \pm  4.2$ \\
Gem_OB1  &  4.00& $12.4 \pm  4.3$ \\
Gem_OB1  &  4.25& $13.4 \pm  3.9$ \\
Gem_OB1  &  4.50& $15.6 \pm  4.1$ \\
Gem_OB1  &  4.75& $16.7 \pm  2.6$ \\
Gem_OB1  &  5.00& $17.4 \pm  2.9$ \\
Gem_OB1  &  5.25& $19.1 \pm  4.4$ \\
Gem_OB1  &  5.50& $19.9 \pm  3.8$ \\
Gem_OB1  &  5.75& $21.3 \pm  3.3$ \\
Gem_OB1  &  7.00& $25.6 \pm  3.2$ \\
Gum_Nebula  &  0.25& $ 0.1 \pm  0.8$ \\
Gum_Nebula  &  0.50& $ 0.4 \pm  0.9$ \\
Gum_Nebula  &  0.75& $ 0.7 \pm  0.9$ \\
Gum_Nebula  &  1.00& $ 0.9 \pm  0.9$ \\
Gum_Nebula  &  1.25& $ 1.0 \pm  1.2$ \\
Gum_Nebula  &  1.50& $ 1.3 \pm  1.2$ \\
Gum_Nebula  &  1.75& $ 1.7 \pm  1.4$ \\
Gum_Nebula  &  2.00& $ 2.2 \pm  1.4$ \\
Gum_Nebula  &  2.25& $ 3.0 \pm  1.8$ \\
Gum_Nebula  &  2.50& $ 4.9 \pm  3.4$ \\
Gum_Nebula  &  2.75& $ 5.4 \pm  3.5$ \\
Gum_Nebula  &  3.00& $ 6.3 \pm  2.1$ \\
Gum_Nebula  &  3.25& $ 7.3 \pm  2.8$ \\
Gum_Nebula  &  3.50& $ 9.0 \pm  6.0$ \\
Hercules  &  0.25& $-0.1 \pm  1.1$ \\
Hercules  &  0.50& $ 1.1 \pm  1.4$ \\
Hercules  &  0.75& $ 3.4 \pm  1.9$ \\
Hercules  &  1.00& $ 4.6 \pm  2.5$ \\
Hercules  &  1.25& $ 6.3 \pm  2.7$ \\
Hercules  &  1.50& $ 9.2 \pm  1.7$ \\
Hercules  &  1.75& $10.5 \pm  1.9$ \\
Hercules  &  2.00& $10.5 \pm  1.8$ \\
Hercules  &  2.25& $10.5 \pm  1.1$ \\
Hercules  &  2.50& $11.6 \pm  4.0$ \\
Lacerta  &  0.25& $ 0.3 \pm  1.0$ \\
Lacerta  &  0.50& $ 1.2 \pm  1.4$ \\
Lacerta  &  0.75& $ 2.8 \pm  1.7$ \\
Lacerta  &  1.00& $ 3.6 \pm  1.8$ \\
Lacerta  &  1.25& $ 4.1 \pm  1.0$ \\
Lupus  &  0.25& $ 0.1 \pm  1.4$ \\
Lupus  &  0.50& $ 0.4 \pm  1.5$ \\
Lupus  &  0.75& $ 1.3 \pm  1.8$ \\
Lupus  &  1.00& $ 2.4 \pm  2.1$ \\
Lupus  &  1.25& $ 3.6 \pm  2.8$ \\
Lupus  &  1.50& $ 5.0 \pm  3.3$ \\
Lupus  &  1.75& $ 6.2 \pm  3.5$ \\
Lupus  &  2.00& $ 8.0 \pm  3.9$ \\
Lupus  &  2.25& $ 9.0 \pm  4.9$ \\
Lupus  &  2.50& $11.7 \pm  4.3$ \\
Lupus  &  2.75& $13.5 \pm  4.8$ \\
Lupus  &  3.00& $15.1 \pm  3.6$ \\
Lupus  &  3.25& $16.9 \pm  5.5$ \\
Lupus  &  3.50& $16.9 \pm  4.1$ \\
Lupus  &  3.75& $19.1 \pm  6.3$ \\
Lupus  &  4.00& $20.3 \pm  7.6$ \\
Lupus  &  4.25& $20.4 \pm  7.6$ \\
Lupus  &  4.50& $18.5 \pm  4.3$ \\
Lupus  &  4.75& $21.1 \pm  7.6$ \\
Lupus  &  5.00& $19.3 \pm  5.9$ \\
Mon_OB1  &  0.25& $ 1.4 \pm  1.7$ \\
Mon_OB1  &  0.50& $ 2.6 \pm  1.9$ \\
Mon_OB1  &  0.75& $ 3.8 \pm  1.9$ \\
Mon_OB1  &  1.00& $ 4.2 \pm  2.8$ \\
Mon_OB1  &  1.25& $ 5.6 \pm  3.8$ \\
Mon_OB1  &  1.50& $ 7.6 \pm  4.5$ \\
Mon_OB1  &  1.75& $ 9.0 \pm  4.0$ \\
Mon_OB1  &  2.00& $10.9 \pm  4.7$ \\
Mon_OB1  &  2.25& $12.5 \pm  4.7$ \\
Mon_OB1  &  2.50& $12.6 \pm  6.5$ \\
Mon_OB1  &  2.75& $13.1 \pm  4.6$ \\
Mon_OB1  &  3.00& $14.1 \pm  3.9$ \\
Mon_OB1  &  3.25& $14.1 \pm  2.0$ \\
Mon_OB1  &  3.50& $16.6 \pm  3.4$ \\
Mon_OB1  &  3.75& $18.2 \pm  4.3$ \\
Mon_OB1  &  4.00& $18.6 \pm  5.2$ \\
Mon_OB1  &  4.25& $20.1 \pm  2.0$ \\
Mon_OB1  &  4.50& $22.0 \pm  2.8$ \\
Mon_OB1  &  6.50& $30.0 \pm  5.4$ \\
Mon_R2  &  0.25& $ 0.2 \pm  1.1$ \\
Mon_R2  &  0.50& $ 0.6 \pm  1.4$ \\
Mon_R2  &  0.75& $ 1.3 \pm  1.5$ \\
Mon_R2  &  1.00& $ 1.9 \pm  1.8$ \\
Mon_R2  &  1.25& $ 2.5 \pm  2.1$ \\
Mon_R2  &  1.50& $ 3.4 \pm  2.7$ \\
Mon_R2  &  1.75& $ 4.7 \pm  3.0$ \\
Mon_R2  &  2.00& $ 6.2 \pm  3.6$ \\
Mon_R2  &  2.25& $ 7.4 \pm  3.8$ \\
Mon_R2  &  2.50& $ 8.9 \pm  4.3$ \\
Mon_R2  &  2.75& $ 9.9 \pm  5.0$ \\
Mon_R2  &  3.00& $11.6 \pm  4.0$ \\
Mon_R2  &  3.25& $13.2 \pm  4.8$ \\
Mon_R2  &  3.50& $12.7 \pm  4.5$ \\
Mon_R2  &  3.75& $15.4 \pm  4.6$ \\
Mon_R2  &  4.00& $14.5 \pm  3.6$ \\
Mon_R2  &  4.25& $16.1 \pm  3.9$ \\
Mon_R2  &  4.50& $17.8 \pm  2.3$ \\
Mon_R2  &  4.75& $16.4 \pm  7.4$ \\
Mon_R2  &  5.00& $17.7 \pm  8.9$ \\
Mon_R2  &  5.25& $16.6 \pm  3.7$ \\
Mon_R2  &  5.75& $21.9 \pm 11.3$ \\
Ophiuchus  &  0.25& $ 0.4 \pm  1.5$ \\
Ophiuchus  &  0.50& $ 0.6 \pm  1.7$ \\
Ophiuchus  &  0.75& $ 0.9 \pm  1.7$ \\
Ophiuchus  &  1.00& $ 1.4 \pm  1.8$ \\
Ophiuchus  &  1.25& $ 2.1 \pm  2.0$ \\
Ophiuchus  &  1.50& $ 3.2 \pm  2.6$ \\
Ophiuchus  &  1.75& $ 3.7 \pm  3.2$ \\
Ophiuchus  &  2.00& $ 5.2 \pm  4.0$ \\
Ophiuchus  &  2.25& $ 6.6 \pm  4.8$ \\
Ophiuchus  &  2.50& $ 7.4 \pm  4.9$ \\
Ophiuchus  &  2.75& $ 9.1 \pm  4.8$ \\
Ophiuchus  &  3.00& $ 8.9 \pm  4.2$ \\
Ophiuchus  &  3.25& $ 9.8 \pm  4.3$ \\
Ophiuchus  &  3.50& $10.4 \pm  4.6$ \\
Ophiuchus  &  3.75& $10.1 \pm  4.3$ \\
Ophiuchus  &  4.00& $10.9 \pm  3.8$ \\
Ophiuchus  &  4.25& $11.6 \pm  4.4$ \\
Ophiuchus  &  4.50& $11.4 \pm  3.6$ \\
Ophiuchus  &  4.75& $13.8 \pm  4.9$ \\
Ophiuchus  &  5.00& $14.0 \pm  2.8$ \\
Ophiuchus  &  5.25& $15.6 \pm  3.4$ \\
Ophiuchus  &  5.50& $16.8 \pm  4.3$ \\
Ophiuchus  &  5.75& $17.3 \pm  3.5$ \\
Ophiuchus  &  6.00& $17.1 \pm  3.9$ \\
Ophiuchus  &  6.50& $17.7 \pm  3.7$ \\
Ophiuchus  &  7.25& $18.8 \pm  1.3$ \\
Ophiuchus  &  8.00& $21.2 \pm  6.7$ \\
Orion_A  &  0.25& $ 0.1 \pm  1.1$ \\
Orion_A  &  0.50& $ 0.5 \pm  1.3$ \\
Orion_A  &  0.75& $ 1.3 \pm  1.7$ \\
Orion_A  &  1.00& $ 2.1 \pm  1.7$ \\
Orion_A  &  1.25& $ 2.6 \pm  2.1$ \\
Orion_A  &  1.50& $ 4.3 \pm  3.2$ \\
Orion_A  &  1.75& $ 5.0 \pm  3.3$ \\
Orion_A  &  2.00& $ 6.7 \pm  3.3$ \\
Orion_A  &  2.25& $ 8.3 \pm  3.3$ \\
Orion_A  &  2.50& $ 8.5 \pm  2.8$ \\
Orion_A  &  2.75& $ 9.4 \pm  2.5$ \\
Orion_A  &  3.00& $10.8 \pm  2.2$ \\
Orion_A  &  3.25& $11.8 \pm  2.8$ \\
Orion_A  &  3.50& $13.0 \pm  3.2$ \\
Orion_A  &  3.75& $14.6 \pm  3.4$ \\
Orion_A  &  4.00& $16.4 \pm  4.8$ \\
Orion_A  &  4.25& $17.0 \pm  5.2$ \\
Orion_A  &  4.50& $17.3 \pm  4.2$ \\
Orion_A  &  4.75& $19.5 \pm  7.7$ \\
Orion_A  &  5.00& $19.9 \pm  4.8$ \\
Orion_A  &  5.25& $16.6 \pm  2.7$ \\
Orion_A  &  5.50& $17.9 \pm  1.9$ \\
Orion_A  &  5.75& $19.9 \pm  3.5$ \\
Orion_A  &  6.00& $20.7 \pm  5.1$ \\
Orion_A  &  6.25& $19.9 \pm  8.1$ \\
Orion_A  &  6.50& $24.7 \pm  8.3$ \\
Orion_A  &  6.75& $21.3 \pm  7.0$ \\
Orion_A  &  7.00& $23.4 \pm  4.6$ \\
Orion_A  &  7.25& $23.9 \pm  3.2$ \\
Orion_A  &  7.50& $18.1 \pm  2.8$ \\
Orion_A  &  7.75& $25.0 \pm  9.7$ \\
Orion_A  &  8.00& $20.7 \pm  6.6$ \\
Orion_A  &  8.25& $23.3 \pm  3.5$ \\
Orion_A  &  8.75& $26.1 \pm 12.9$ \\
Orion_A  &  9.25& $29.8 \pm 10.1$ \\
Orion_A  &  9.75& $29.4 \pm  7.4$ \\
Orion_A  & 11.00& $34.6 \pm  5.0$ \\
Orion_A  & 11.25& $31.7 \pm  8.7$ \\
Orion_A  & 11.50& $36.0 \pm  4.8$ \\
Orion_A  & 11.75& $31.7 \pm  2.8$ \\
Orion_A  & 12.75& $42.3 \pm  8.1$ \\
Orion_A  & 15.00& $32.0 \pm  7.0$ \\
Orion_B  &  0.25& $ 0.6 \pm  1.2$ \\
Orion_B  &  0.50& $ 1.3 \pm  1.5$ \\
Orion_B  &  0.75& $ 2.1 \pm  1.9$ \\
Orion_B  &  1.00& $ 3.4 \pm  2.4$ \\
Orion_B  &  1.25& $ 4.4 \pm  3.3$ \\
Orion_B  &  1.50& $ 5.2 \pm  3.2$ \\
Orion_B  &  1.75& $ 6.4 \pm  3.4$ \\
Orion_B  &  2.00& $ 7.9 \pm  3.8$ \\
Orion_B  &  2.25& $ 9.3 \pm  3.6$ \\
Orion_B  &  2.50& $ 9.9 \pm  4.0$ \\
Orion_B  &  2.75& $12.4 \pm  3.9$ \\
Orion_B  &  3.00& $13.0 \pm  4.0$ \\
Orion_B  &  3.25& $16.1 \pm  5.6$ \\
Orion_B  &  3.50& $17.8 \pm  3.5$ \\
Orion_B  &  3.75& $20.9 \pm  6.8$ \\
Orion_B  &  4.00& $21.2 \pm  8.1$ \\
Orion_B  &  4.25& $23.3 \pm  9.5$ \\
Orion_B  &  4.50& $26.5 \pm  9.9$ \\
Orion_B  &  4.75& $22.6 \pm 10.1$ \\
Orion_B  &  5.00& $32.7 \pm  8.5$ \\
Orion_B  &  5.25& $36.8 \pm 12.8$ \\
Orion_B  &  5.75& $35.2 \pm 10.4$ \\
Orion_B  &  6.25& $41.4 \pm 16.8$ \\
Orion_B  &  6.50& $36.4 \pm 16.5$ \\
Orion_B  &  6.75& $41.2 \pm 14.8$ \\
Pipe_Nebula  &  0.25& $ 1.5 \pm  2.0$ \\
Pipe_Nebula  &  0.50& $ 2.7 \pm  2.4$ \\
Pipe_Nebula  &  0.75& $ 3.5 \pm  2.5$ \\
Pipe_Nebula  &  1.00& $ 3.2 \pm  2.6$ \\
Pipe_Nebula  &  1.25& $ 3.5 \pm  2.5$ \\
Pipe_Nebula  &  1.50& $ 4.1 \pm  2.8$ \\
Pipe_Nebula  &  1.75& $ 5.3 \pm  2.4$ \\
Pipe_Nebula  &  2.00& $ 6.5 \pm  2.6$ \\
Pipe_Nebula  &  2.25& $ 7.8 \pm  2.5$ \\
Pipe_Nebula  &  2.50& $ 9.1 \pm  2.8$ \\
Pipe_Nebula  &  2.75& $11.0 \pm  2.9$ \\
Pipe_Nebula  &  3.00& $12.2 \pm  3.3$ \\
Pipe_Nebula  &  3.25& $15.7 \pm  2.7$ \\
Pipe_Nebula  &  3.50& $15.3 \pm  4.7$ \\
Pipe_Nebula  &  3.75& $17.1 \pm  4.0$ \\
Pipe_Nebula  &  4.00& $18.1 \pm  3.1$ \\
Pipe_Nebula  &  4.25& $19.1 \pm  2.5$ \\
Pipe_Nebula  &  4.50& $19.9 \pm  2.4$ \\
Pipe_Nebula  &  4.75& $21.3 \pm  2.5$ \\
Pipe_Nebula  &  5.25& $20.0 \pm  7.7$ \\
Pegasus  &  0.25& $ 0.4 \pm  1.0$ \\
Pegasus  &  0.50& $ 1.9 \pm  1.5$ \\
Pegasus  &  0.75& $ 4.1 \pm  2.2$ \\
Pegasus  &  1.00& $ 6.9 \pm  1.7$ \\
Pegasus  &  1.25& $ 8.5 \pm  2.8$ \\
Perseus  &  0.25& $ 0.7 \pm  1.5$ \\
Perseus  &  0.50& $ 1.4 \pm  1.9$ \\
Perseus  &  0.75& $ 2.5 \pm  2.2$ \\
Perseus  &  1.00& $ 3.7 \pm  3.0$ \\
Perseus  &  1.25& $ 5.9 \pm  3.4$ \\
Perseus  &  1.50& $ 6.9 \pm  3.6$ \\
Perseus  &  1.75& $ 8.4 \pm  3.1$ \\
Perseus  &  2.00& $10.3 \pm  3.2$ \\
Perseus  &  2.25& $12.0 \pm  4.5$ \\
Perseus  &  2.50& $14.0 \pm  5.1$ \\
Perseus  &  2.75& $15.5 \pm  4.2$ \\
Perseus  &  3.00& $16.8 \pm  3.9$ \\
Perseus  &  3.25& $17.8 \pm  6.7$ \\
Perseus  &  3.50& $20.6 \pm  7.1$ \\
Perseus  &  3.75& $19.9 \pm  4.2$ \\
Perseus  &  4.00& $21.6 \pm  4.3$ \\
Perseus  &  4.25& $20.4 \pm  4.3$ \\
Perseus  &  4.50& $21.6 \pm  4.9$ \\
Perseus  &  4.75& $25.0 \pm  7.5$ \\
Perseus  &  5.00& $26.3 \pm  5.2$ \\
Perseus  &  5.25& $25.8 \pm  7.7$ \\
Perseus  &  5.50& $25.4 \pm  7.7$ \\
Perseus  &  5.75& $28.0 \pm  7.8$ \\
Perseus  &  6.00& $29.7 \pm  6.5$ \\
Perseus  &  6.50& $29.2 \pm  5.0$ \\
Perseus  &  6.75& $28.0 \pm  8.4$ \\
Perseus  &  7.00& $28.8 \pm  7.9$ \\
Polaris_Flare  &  0.25& $ 0.5 \pm  1.0$ \\
Polaris_Flare  &  0.50& $ 1.5 \pm  1.4$ \\
Polaris_Flare  &  0.75& $ 2.8 \pm  2.5$ \\
Polaris_Flare  &  1.00& $ 4.3 \pm  2.9$ \\
Polaris_Flare  &  1.25& $ 5.0 \pm  2.8$ \\
Polaris_Flare  &  1.50& $ 5.6 \pm  2.2$ \\
Polaris_Flare  &  1.75& $ 5.7 \pm  2.7$ \\
R_Coronae_Australis  &  0.25& $-0.1 \pm  1.2$ \\
R_Coronae_Australis  &  0.50& $ 0.5 \pm  1.3$ \\
R_Coronae_Australis  &  0.75& $ 2.4 \pm  1.7$ \\
R_Coronae_Australis  &  1.00& $ 4.7 \pm  1.8$ \\
R_Coronae_Australis  &  1.25& $ 5.9 \pm  2.2$ \\
R_Coronae_Australis  &  1.50& $ 7.1 \pm  1.9$ \\
R_Coronae_Australis  &  1.75& $ 8.4 \pm  2.7$ \\
R_Coronae_Australis  &  2.00& $10.0 \pm  2.3$ \\
R_Coronae_Australis  &  2.25& $ 9.4 \pm  1.5$ \\
R_Coronae_Australis  &  2.50& $ 9.4 \pm  1.3$ \\
R_Coronae_Australis  &  3.25& $13.7 \pm  5.5$ \\
Rosette  &  0.25& $ 1.4 \pm  1.0$ \\
Rosette  &  0.50& $ 1.5 \pm  1.5$ \\
Rosette  &  0.75& $ 2.2 \pm  1.9$ \\
Rosette  &  1.00& $ 2.6 \pm  2.0$ \\
Rosette  &  1.25& $ 2.1 \pm  1.6$ \\
Rosette  &  1.50& $ 2.2 \pm  1.3$ \\
Rosette  &  1.75& $ 3.0 \pm  1.7$ \\
Rosette  &  2.00& $ 3.4 \pm  1.5$ \\
Rosette  &  2.25& $ 3.7 \pm  1.8$ \\
Rosette  &  2.50& $ 4.9 \pm  2.9$ \\
Rosette  &  2.75& $ 4.9 \pm  2.1$ \\
Rosette  &  3.00& $ 6.4 \pm  3.0$ \\
Rosette  &  3.25& $ 5.3 \pm  1.7$ \\
Rosette  &  3.50& $ 7.0 \pm  1.8$ \\
Rosette  &  3.75& $ 8.2 \pm  1.8$ \\
Rosette  &  4.00& $ 8.7 \pm  2.5$ \\
Rosette  &  4.25& $ 9.2 \pm  3.0$ \\
Rosette  &  4.50& $10.3 \pm  2.8$ \\
Rosette  &  4.75& $10.7 \pm  2.5$ \\
Rosette  &  5.25& $13.3 \pm  3.0$ \\
Rosette  &  5.50& $12.6 \pm  5.8$ \\
Rosette  &  6.00& $14.8 \pm  1.2$ \\
Rosette  &  6.25& $14.8 \pm  2.1$ \\
Rosette  &  6.50& $14.3 \pm  1.7$ \\
Taurus  &  0.25& $ 1.8 \pm  2.0$ \\
Taurus  &  0.50& $ 2.8 \pm  2.7$ \\
Taurus  &  0.75& $ 3.8 \pm  3.8$ \\
Taurus  &  1.00& $ 5.7 \pm  3.7$ \\
Taurus  &  1.25& $ 6.8 \pm  3.1$ \\
Taurus  &  1.50& $ 7.5 \pm  3.7$ \\
Taurus  &  1.75& $ 8.0 \pm  3.2$ \\
Taurus  &  2.00& $ 9.1 \pm  3.5$ \\
Taurus  &  2.25& $ 9.8 \pm  3.0$ \\
Taurus  &  2.50& $10.7 \pm  3.3$ \\
Taurus  &  2.75& $11.2 \pm  2.7$ \\
Taurus  &  3.00& $12.0 \pm  3.6$ \\
Taurus  &  3.25& $12.6 \pm  3.3$ \\
Taurus  &  3.50& $13.1 \pm  3.5$ \\
Taurus  &  3.75& $13.0 \pm  2.9$ \\
Taurus  &  4.00& $14.0 \pm  2.5$ \\
Taurus  &  4.25& $14.1 \pm  2.9$ \\
Taurus  &  4.50& $14.1 \pm  2.4$ \\
Taurus  &  4.75& $14.9 \pm  3.6$ \\
Taurus  &  5.00& $15.3 \pm  2.5$ \\
Taurus  &  5.25& $15.1 \pm  4.1$ \\
Taurus  &  5.50& $15.4 \pm  4.0$ \\
Taurus  &  5.75& $17.3 \pm  3.5$ \\
Taurus  &  6.00& $16.6 \pm  3.2$ \\
Taurus  &  6.25& $18.1 \pm  5.1$ \\
Taurus  &  6.50& $18.3 \pm  4.2$ \\
Taurus  &  6.75& $16.5 \pm  2.3$ \\
Taurus  &  7.00& $17.0 \pm  3.0$ \\
Taurus  &  7.25& $17.3 \pm  6.7$ \\
Taurus  &  7.75& $19.6 \pm  2.6$ \\
Taurus  &  8.00& $17.0 \pm  2.7$ \\
Taurus  &  8.50& $19.9 \pm  1.5$ \\
\hline \hline
\end{tabular}

